Probabilistic Models with Deep Neural Networks

Recent advances in statistical inference have significantly expanded the toolbox of probabilistic modeling. Historically, probabilistic modeling has been constrained to (i) very restricted model classes where exact or approximate probabilistic inference were feasible, and (ii) small or medium-sized data sets which fit within the main memory of the computer. However, developments in variational inference, a general form of approximate probabilistic inference originated in statistical physics, are allowing probabilistic modeling to overcome these restrictions: (i) Approximate probabilistic inference is now possible over a broad class of probabilistic models containing a large number of parameters, and (ii) scalable inference methods based on stochastic gradient descent and distributed computation engines allow to apply probabilistic modeling over massive data sets. One important practical consequence of these advances is the possibility to include deep neural networks within a probabilistic model to capture complex non-linear stochastic relationships between random variables. These advances in conjunction with the release of novel probabilistic modeling toolboxes have greatly expanded the scope of application of probabilistic models, and allow these models to take advantage of the recent strides made by the deep learning community. In this paper we review the main concepts, methods and tools needed to use deep neural networks within a probabilistic modeling framework.

==> hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for � markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\boldsymbol{\Upsilon}$}}}
\nc{\bmupsilon}{{\mbox{\bm $\boldsymbol{\upsilon}$}}}
\nc{\bmalpha}{{\mbox{\bm $\boldsymbol{\alpha}$}}}
\nc{\bmbeta}{{\mbox{\bm $\boldsymbol{\beta}$}}}
\nc{\bmgamma}{{\mbox{\bm $\boldsymbol{\gamma}$}}}
\nc{\bmGamma}{{\mbox{\bm $$\boldsymbol{\Gamma}$}}}
\nc{\bmdelta}{{\mbox{\bm $\boldsymbol{\delta}$}}}
\nc{\bmDelta}{{\mbox{\bm $\boldsymbol{\Delta}$}}}
\nc{\bmeps}{{\mbox{\bm $\boldsymbol{\epsilon}$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\boldsymbol{\phi}$}}}
\nc{\bmPhi}{{\mbox{\bm $\$\boldsymbol{\Phi}$}}}
\nc{\bmlambda}{{\mbox{\bm $\boldsymbol{\lambda}$}}}
\nc{\bmLambda}{{\mbox{\bm $\boldsymbol{\Lambda}$}}}
\nc{\bmmu}{{\mbox{\bm $\boldsymbol{\mu}$}}}
\nc{\bmnu}{{\mbox{\bm $\boldsymbol{\nu}$}}}
\nc{\bmpi}{{\mbox{\bm $\boldsymbol{\pi}$}}}
\nc{\bmrho}{{\mbox{\bm$\boldsymbol{\rho}$}}}
\nc{\bmpsi}{{\mbox{\bm $\boldsymbol{\psi}$}}}
\nc{\bmPsi}{{\mbox{\bm $\boldsymbol{\Psi}$}}}
\nc{\bmsigma}{{\mbox{\bm $$\boldsymbol{\sigma}$}}}
\nc{\bmSigma}{{\mbox{\bm $\boldsymbol{\Sigma}$}}}
\nc{\bmtheta}{{\ensuremath{\boldsymbol{\theta}}}}
%\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
\nc{\bmeta}{{\ensuremath{\boldsymbol{\eta}}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}


==> model-PCA-mixed.tex <==
% !TEX root = texmain.tex
\section{Probabilistic Modeling within the Conjugate Exponential Family}\label{sec:models}
In the first subsection we introduce notation and present conjugate exponential family and latent variable models (LVMs).
In the second subsection, we detail how to apply variational inference methods to fit LVMs from data. Finally, we show how to
scale variational methods to learn LVMs over massive data sets.

\subsection{Latent Variable Models}
\label{sec:LVM}

Principal Component Analysis (PCA) is a classic statistical technique for dimensionality reduction. We consider this model as a running example to better understand the content of the paper. PCA maps a d-dimensional point $\bmx$ to a k-dimensional latent representation $\bmz$ through a affine matrix $\bmbeta$ of dimensions $d\times k$. A (simplified) probabilistic view of PCA \citep{tipping1999probabilistic} can be described by the following generative process, 
\begin{equation}\label{eq:pca}
\begin{split}
%\bmalpha = (\sigma_\beta, \sigma_z, \sigma_x)\nonumber\\
\bmbeta \sim \calN_{d\times k} (0,\bmI\sigma^2_\beta) \nonumber\\ 
\bmz_i \sim \calN_k (0,\bmI)\nonumber\\ 
\bmx_i \sim \calN_d (\bmbeta^T\bmz_i, \sigma^2_x\bmI ),
\end{split}
\end{equation}
\noindent where $\bmalpha = (\sigma^2_\beta, \sigma^2_x)$ are the hyperparameters of the model. 

This model is an example of a latent variable model (LVM) \citep{bishop1998latent,blei2014build}. LVMs 
are widely used probabilistic models which tries to uncover hidden patterns in our data set. These hidden 
patterns are modeled by means of a global hidden random variable, denoted by $\bmbeta$, which captures hidden quantities common all 
the observations. And by a set of local hidden stochastic 
random variables, denoted by $\bmz_i$, which capture hidden pattern specific for each observation. The observed data, denoted by $\bmx$, 
is assumed to be generated from stochastic random variables whose distribution is conditioned to both the 
local and global hidden variables. A vector of fixed (hyper) parameters denoted by $\bmalpha$ is also included in this kind of models. The general structure 
of this model is depicted in \figref{plateModel}. In the case of the PCA model, $\bmbeta$ acts as the global hidden variable encoding the possible affine matrices, and $\bmz_i$ are the local hidden variables associated to the sample $\bmx_i$ encoding the low-dimensional representation of each data sample.


The joint distribution of these probabilistic models factorizes into a product of local terms and a global term, 
\[
p(\bmx, \bmz, \bmbeta)  = p(\bmbeta) \prod_{i=1}^N p(\bmx_i, \bmz_i|\bmbeta).
\]

Another assumption employed in this kind of models is that they belong to the conjugate exponential family \citep{barndorff2014information}. 
The conjugate exponential family has been largely studied in the statistics field and cover a very wide 
and widely used range of probability distributions and density functions such as Multinomial, 
Normal, Gamma, Dirichlet, Beta, etc. They have been largely used by the machine learning community \citep{bishop2006pattern,koller2009probabilistic,murphy2012machine}  
to exploit many of their nice properties for parameter learning and inference tasks. 

As a LVM is assumed to belongs to the conjugate exponential family, the functional form of the conditional distributions of the model can be specified as follows,  
\begin{eqnarray}\label{eq:model}
\ln p(\bmbeta) &=& \ln h(\bmbeta) + \bmalpha^T t(\bmbeta) - a_g(\bmalpha)\nonumber\\
\ln p(\bmz_i|\bmbeta) &=& \ln h(\bmz_i)  + \eta_z(\bmbeta)^T t(\bmz_i) - a_z(\eta_z(\bmbeta))\nonumber\\
\ln p(\bmx_i|\bmz_i,\bmbeta) &=& \ln h(\bmx_i)  + \eta_x(\bmz_i,\bmbeta)^T t(\bmx_i) - \eta_x(\bmz_i,\bmbeta)),
\end{eqnarray}
\noindent where the scalar functions $h(\cdot)$ and $a_l(\cdot)$ are the base measure and the log-normalizer,
respectively; the vector function $\bmt(\cdot)$ is the \textit{sufficient statistics} vector.

By using properties of the conjugate exponential family, we can also derived the functional form of the joint distributions over the local variables $(\bmz_i,\bmx_i)$ given the global parameters $\bmbeta$,
\begin{equation}\label{eq:jointexponentialform}
\ln p(\bmx_i,\bmz_i|\bmbeta) = \ln h(\bmx_i,\bmz_i) + \bmbeta^{T} t(\bmx_i,\bmz_i) - a_l(\bmbeta),
\end{equation}
%\noindent where the scalar functions $h(\cdot)$ and $a_l(\cdot)$ are the base measure and the log-normalizer,
%respectively; the vector function $\bmt(\cdot)$ is the \textit{sufficient statistics} vector. And, similarly, for the prior distribution $p(\bmbeta)$, 
%\begin{equation}\label{eq:priormodel}
%\ln p(\bmbeta\given\bmalpha) = \ln h(\bmbeta) + \bmalpha^T t(\bmbeta) - a_g(\bmalpha)
%\end{equation}

Another standard assumption \citep{HoffmanBleiWangPaisley13} in this kind of models is that the \textit{complete conditional} forms of the latent variables given the observations and the other latent variables can also be expressed in exponential family form, 
\begin{equation}\label{eq:posteriorexponentialform}
\begin{split}
\ln p(\bmbeta|\bmx, \bmz) = h(\bmbeta)  + \eta_g(\bmx, \bmz)^T t(\bmbeta) - a_g(\eta_g(\bmx, \bmz))\\
\ln p(\bmz_i|\bmx_i, \bmbeta) = h(\bmz_i)  + \eta_l(\bmx_i,\bmbeta)^T t(\bmz_i) - a_l(\eta_l(\bmx_i,\bmbeta)).
\end{split}
\end{equation}

By conjugacy properties, the natural parameter of the global posterior $\eta_g(\bmx, \bmz)$ can be expressed as, 
\begin{equation}\label{eq:naturalglobal}
\eta_g(\bmx, \bmz) = \bmalpha + \sum_{i=1}^N t(\bmx_i,\bmz_i)
\end{equation}

The probabilistic PCA model belongs to the conjugate exponential family because its generative model (see Equations~\eqref{eq:pca}) can be expressed in terms of the functional forms described in Equation~\eqref{eq:model}, and it also satisfies the \textit{complete conditional} assumptions because both $p(\bmbeta|\bmx,\bmz)$ and $p(\bmz_i|\bmx_i,\bmz)$ are both multivariate normal distribution \citep{tipping1999probabilistic}. However, note that the linear relationship between the hidden and the observed variables are a strong limitation of this model \citep{scholkopf1998nonlinear}. Also note that this linear relationship is made to guarantee that the PCA model belongs to conjugate exponential family. The use of any other non-linear relationship would make the PCA model to not belong to this family and would prevent, as we will see in the next section, the use of efficient inference algorithms. Something similar happens with the variance parameter $\sigma_x$, which can not depend on the latent variables $\bmz_i$ in order to belong to the conjugate exponential family.

LVMs considered in this section also include popular models like LDA models \citep{blei2003latent} to uncover the hidden topics in a text corpora, mixture of Gaussian models to discover hidden clusters in our data \citep{bishop2006pattern}, probabilistic principal component analysis for revealing a low-dimensional representation of the data \citep{tipping1999probabilistic}, models with hierarchical latent variables to capture the drift in a data stream \citep{borchani2015modeling,masegosa2017bayesian}, etc. Many machine-learning books contain entire sections devoted to them \citep{bishop2006pattern,koller2009probabilistic,murphy2012machine}.


%As shown in \citep{WinnBishop05,HoffmanBleiWangPaisley13}, we can also express the conditional distributions in this alternative parametrization, 
%\begin{equation}\label{eq:Fexponentialform}
%\begin{split}
%& \ln p(\bmy|\Pa(\bmy)) = h_\bmy(\bmy)  + \eta_{\bmy}^T \bmt (\bmy,\Pa(\bmy)) - a_{\bmy}(\eta_\bmy),
%\end{split}
%\end{equation}
%
%Using the above parameterization, we can express the joint probability distribution as follows, 
%\begin{equation}\label{eq:jointexponentialform}
%\begin{split}
%& \ln p(\bmx, \bmz, \bmbeta) = h(\bmx,\bmz, \bmbeta)  + \eta^T \bmt(\bmx, \bmz, \bmbeta) - a(\bmx, \bmz, \bmbeta),
%\end{split}
%\end{equation}
%\noindent where $\eta_{\bmx}$ and $\bmt_\bmx(\bmx)$ are defined simply by concatenating the natural parameters $\eta_{Y}$ 
%and the sufficient statistics $\bmt(Y,\Pa(Y))$ for all the random variables of the model, respectively. Similarly,  $a_{\bmx}(\eta_\bmx)$ and $h_\bmx(\bmx)$ are defined as the sum of the individual log-base measures $h_Y(\cdot)$ and log-normalizers functions, $a_Y(\cdot)$, respectively. See \citep{WinnBishop05,HoffmanBleiWangPaisley13} for further details. 
%
%Because this model is conjugate exponential family model we can express in similar terms the posterior probability over $\bmbeta$ as follows \citep{WinnBishop05,HoffmanBleiWangPaisley13}, 
%\begin{equation}\label{eq:posteriorexponentialform}
%\begin{split}
%\ln p(\bmbeta|\bmx, \bmz) = h_\bmbeta(\bmbeta)  + \eta_\bmbeta(\bmx, \bmz)^T \bmt_\bmbeta(\bmbeta) - a_\bmbeta(\bmx, \bmz)\\
%= h_\bmbeta(\bmbeta)  + \sum_{i=1}^N \eta_\bmbeta(\bmx_i, \bmz_i)^T \bmt_\bmbeta(\bmbeta) - a_\bmbeta(\bmx_i, \bmz_i),
%\end{split}
%\end{equation}
%
%For the model of Figure \ref{fig:plateModel}, we have that $\bmz_i$ is independent from $\bmz_j$ (with $i\neq j$) given $\bmbeta$. In consequence, the posterior over $\bmz_i$ can be expressed as $p(\bmz_i|\bmx_i, \bmbeta)$. By conjugacy rules, this posterior can also be expressed as, 
%\begin{equation}\label{eq:posteriorexponentialform:local}
%\begin{split}
%\ln p(\bmz_i|\bmx_i, \bmz) = h(\bmz_i)  + \eta_{z_i}(\bmx_i,\bmbeta)^T \bmt_{z_i}(\bmz_i) - a_{z_i}(\bmx_i,\bmbeta)
%\end{split}
%\end{equation}
%These nice transformations are possible because Equation~(\ref{eq:jointexponentialform}) can be really expressed as a multi-linear function of the sufficient statistics $\bmt_Y$ of the random variables of the model \citep{WinnBishop05}. In that way, we can see that a conjugate exponential family model maps the random variables to an alternative representation space, through the sufficient statistics function $\bmt(\cdot)$, and, once there, the log joint probability distributions is expressed as a (multi)-linear function. 

%This simple functional form of conjugate exponential family models made them very amenable for many tasks, especially for variational inference as we will see in the next subsection. However, when the variables involved in the probabilistic model does not have a simple linear dependency relationship, as happens when modeling the pixels of an image, the words within a corpus, etc., conjugate exponential family models are not powerful enough. 
%
%
%
%\begin{exmp}\label{example:PCA}
%Principal Component Analysis (PCA) is a classic statistical technique for dimensionality reduction. It maps a d-dimensional point $\bmx$ to a k-dimensional latent representation $\bmz$ through a affine matrix $\bmbeta$ of dimensions $d\times k$. A simplified probabilistic view of PCA \citep{tipping1999probabilistic} can be describe as follows, 
%\begin{equation}\label{eq:pca}
%\begin{split}
%%\bmalpha = (\sigma_\beta, \sigma_z, \sigma_x)\nonumber\\
%\bmbeta \sim \calN_{d\times k} (0,\bmI\sigma^2_\beta) \nonumber\\ 
%\bmz_i \sim \calN_k (0,\bmI)\nonumber\\ 
%\bmx_i \sim \calN_d (\bmbeta^T\bmz_i, \bmI\sigma^2_x ),
%\end{split}
%\end{equation}
%\noindent where $\bmalpha = (\sigma^2_\beta, \sigma^2_x)$ are the hyperparameters of the model. 
%
%This model is a LVM where $\bmbeta$ acts a the global hidden variable and $\bmz_i$ is the local hidden variables associated to the sample $\bmx_i$. It belongs to the conjugate exponential family because all the conditionals are Gaussian distributions whose the mean is expressed as a linear combination of preceding variables \cite{koller2009probabilistic}. Therefore, they satisfy Equation~(\ref{eq:model}). 

%and with the following natural parameters, 
%\begin{equation*}\label{eq:pcaNatural}
%\begin{split}
%\bmalpha = \begin{bmatrix} \frac{1}{\sigma_\beta}\mathbf{0} \\ \frac{-1}{2\sigma_\beta}\bmI\end{bmatrix} & 
%\quad \eta_{\bmx_i}(\bmz_i,\bmbeta) = \begin{bmatrix} \frac{1}{\sigma_x}\bmbeta^T\bmz_i \\ \frac{-1}{2\sigma_x}\bmI\end{bmatrix} \\
%\eta_\bmbeta(\bmx,\bmz) = \begin{bmatrix} \\ \end{bmatrix} &
%\quad \eta_{z_i}(\bmx_i,\bmbeta) = \begin{bmatrix} \\ \end{bmatrix}
%\end{split}
%\end{equation*}
%Note that this linear relationship between the hidden and the observed variables is a strong limitation of this model. Also note this linear relationship is made to guarantee that the model belongs to conjugate exponential family. The use of any other non-linear relationship would make the PCA model to not belong to this family and would prevent, as we will see in the next section, the use of efficient inference algorithms. Something similar happens with the variance parameter $\sigma_x$, which can not depend on the latent variables $\bmz_i$ in order to belong to the conjugate exponential family.
%\end{exmp}



\subsection{Mean-Field Variational Inference}\label{sec:VI}

The problem of Bayesian inference reduces to compute the posterior over the unknown quantities (i.e. the global and local hidden variables $\bmbeta$ and $\bmz$, respectively) given the observations, 

\begin{equation} \label{eq:VI}
p(\bmbeta, \bmz\given \bmx) = \frac{p(\bmx|\bmz,\bmbeta)p(\bmz\given \bmbeta)p(\bmbeta)}{\int p(\bmx|\bmz,\bmbeta)p(\bmz\given \bmbeta)p(\bmbeta) d\bmz d\bmbeta}.
\end{equation}
Computing the above posterior is usually intractable for many interesting models because it requires to solve a highly-multidimensional integral. As commented in the in the introduction, VI methods are one of the best performing options to address this problem. In this section we revise the main ideas behind this approach. 

Variational inference is a deterministic
technique for finding tractable posterior distributions, denoted by $q$, which approximates the Bayesian
posterior,  $p(\bmbeta,\bmz|\bmx)$, that is often intractable to compute. More specifically, by letting ${\cal Q}$
be a set of possible approximations of this posterior, variational inference solves the following optimization problem for any model in the conjugate exponential family:
\begin{equation} \label{eq:VIKL}
\min_{q\left(\bmbeta,\bmz\right)\in {\cal Q}} \KL(q(\bmbeta,\bmz)||p(\bmbeta,\bmz|\bmx)),
\end{equation}
\noindent where $\KL$ denotes the Kullback-Leibler divergence between two probability distributions. 


\begin{figure}
\begin{center}
\scalebox{0.95}{
\begin{tikzpicture}
  % Define nodes
  % Beta
  \node[latent]  (beta)   {$\boldsymbol{\beta}$}; %
  
  % alpha
  \node[const, left= .5  of beta]  (alpha)   {$\bmalpha$}; %
  \edge{alpha}{beta};
  
  % X
  \node[obs, below right=1 of beta]          (X)   {$\bmx_{i}$}; %
  \edge{beta}{X};
 
  % Z
  \node[latent, below left= 1 of beta]          (Z)   {$\bmz_{i}$}; %
  \edge{Z}{X};
  \edge{beta}{Z};
  
  % Plates
  \plate {Observations} { %
    (X)(Z)
  } {\tiny $i={1,\ldots, N}$} ;

%  \plate {time} { %
%    (X)(Z)(beta)(Observations)
%  } {\tiny $t={1,\ldots, T}$} ;


\end{tikzpicture}
}

\end{center}
\vspace{-3mm}
\caption{\label{fig:plateModel} Core of the probabilistic model examined in this paper. See Section \secref{sec:LVM} for details.}
\end{figure}

In the \textit{mean field variational} approach the approximation family ${\cal Q}$ is assumed to fully factorize, i.e. $q\left(\bmbeta,\bmz\right) = q(\bmbeta)\prod_{i=1}^N q(\bmz_i)$. By the \textit{calculus of variations} (hence the name "variational Bayes"), a solution to minimizing the KL divergence, as described in Equation~\eqref{a}, can be found by iteratively applying the following set of updating equations,
\begin{eqnarray*}
\ln q(\bmbeta) =  \E_{q\neq q(\beta)} [\ln p(\bmx, \bmz, \bmbeta)] + cte\\
\ln q(\bmz_i) =  \E_{q\neq q(z_i)} [\ln p(\bmx_i,\bmz_i,\bmbeta)] + cte,
\end{eqnarray*}
\noindent where $\E_{q\neq q(\beta)}[\cdot]$ and $\E_{q\neq q(z_i)}[\cdot]$ denote expectation according to all the $q$ factors expect  $q(\bmbeta)$ and $q(\bmz_i)$, respectively. 

In the case of the probabilistic PCA running example, the variational distribution family would be specified as, $q(\bmbeta\given \bmmu_{\beta},  \mathbf{\Sigma}_{\beta}) = {\cal N}_{d\times k}(\bmmu_{\beta},  \mathbf{\Sigma}_{\beta})$ and $q(\bmz_i \given \bmmu_{z,i}, \mathbf{\Sigma}_{z,i}) = \prod_{i=1}^N {\cal N}_{k}(\bmmu_{z,i},   \mathbf{\Sigma}_{z,i})$. And the coordinate updating equations could be written in closed-form as follows \citep{bishop2006pattern},
\begin{eqnarray*}
\bmmu_{\beta}^\star &=& \big[\sum_{i=1}^N (\bmx_i - \bar{\bmx})\E[\bmz_i]^T\big]\mathbf{\Sigma}_{\beta}\\
\mathbf{\Sigma}_{\beta}^\star &=& \sum_{i=1}^N \E[\bmz_i\bmz_i^T] +  \sigma_x A)\\
\bmmu_{z,i}^\star &=& \sigma_x^2 \mathbf{\Sigma}_{z,i}^{-1}\bmmu_{\beta}^T(\bmx_i -\bar{\bmx})\\
\mathbf{\Sigma}_{z,i}^\star &=& \sigma_x^{-2}\bmmu_{\beta}^T\bmmu_{\beta} + \bmI
\end{eqnarray*}  
\noindent where $A$ is a diagonal matrix with elements $\alpha_i = \frac{d}{\bmmu_{\beta,i}^T\bmmu_{\beta,i}}$.
As we can see, PCA has a nice set of close-form equations which guarantees convergence to the solution of the inference problem. But we should note that this is possible due to the strong assumptions imposed to the probabilistic model and to the variational approximation family. 

\subsection{Mean-Field Variational Inference for conjugate exponential models}
The question is that the above updating variational equations 

%\footnote{More general mean-field approximations can also be used \citep{WinnBishop05}.}
Following the notation of \citet{HoffmanBleiWangPaisley13}, we have that
\[
q(\bmbeta,\bmz\given \bmlambda,\bmphi) = q(\bmbeta \given \bmlambda)\prod_{i=1}^N  q(\bmz_i \given \bmphi_i).
\] 
\noindent where $\bmlambda$ parameterizes the variational distribution of $\bmbeta$, while $\bmphi$ has the same role for the variational distribution of $\bmz$
%where $J$ is the number of local hidden variables, which is assumed fixed for all $i=1,\ldots, N$. 

Furthermore, each factor in the variational distribution is assumed to belong to the same family of the model's \textit{complete conditionals} (see Equation~\eqref{eq:posteriorexponentialform}), 
\begin{equation*}\label{eq:qexponentialform}
\begin{split}
\ln q(\bmbeta|\bmlambda) = h(\bmbeta)  + \bmlambda^T t(\bmbeta) - a_g(\bmlambda)\\
\ln q(\bmz_i|\bmphi_i) = h(\bmz_i)  + \bmphi_i^T t(\bmz_i) - a_l(\bmphi_i).
\end{split}
\end{equation*}

To solve the minimization problem in Equation (\ref{eq:VI}), the variational approach exploits  the  transformation
\begin{equation}
  \label{eq:likelihood_decomposition}
\ln p(\bmx) = {\cal L}(\bmlambda,\bmphi) + \KL(q(\bmbeta,\bmz\given \bmlambda,\bmphi)||p(\bmbeta,\bmz|\bmx)),  
\end{equation}
\noindent where ${\cal L}(\cdot|\cdot)$ is a \emph{lower bound} of $\ln P(\bmx)$ since $\KL$ is  non-negative. 
As  $\ln p(\bmx)$ is constant, minimizing the $\KL$ term is equivalent to maximizing the lower bound. Variational methods maximize this lower bound by using gradient based methods. 

%applying a coordinate  ascent that iteratively updates the individual variational distributions while holding the others fixed~\citep{WinnBishop05}. 

The functional form of the $\lb$ function can expressed as follows, 
\begin{equation}\label{eq:elbo}
\begin{split}
{\cal L}(\bmlambda,\bmphi)  = & \E_q [\ln p(\bmx, \bmz, \bmbeta)] - \E_q [\ln q(\bmbeta,\bmz|\bmlambda,\bmphi)]\\
\end{split}
\end{equation}
%= &\sum_{i=1}^N (\E_q [\ln p(\bmx, \bmz_i|\bmbeta)]  - \E_q [\ln q(\bmz_i|\bmphi)]) \\
%  & + \E_q [\ln p(\bmbeta)] - \E_q [\ln q(\bmbeta|\bmlambda)]\\

The key advantage of having a conjugate exponential model is that the gradients of the $\lb$ function can be always computed in closed form ~\citep{WinnBishop05}. The gradients 
with respect to the variational parameters $\bmlambda$ and $\bmphi$ can be computed as follows, 
\begin{equation}\label{eq:gradELBO}
\begin{split}
\nabla^{nat}_\lambda {\cal L} (\bmlambda,\bmphi) &= \bmalpha + \sum_{i=1}^N  \E_{\phi_i} [t(\bmx_i,\bmz_i)]  - \bmlambda\\
\nabla^{nat}_{\phi_i}{\cal L} (\bmlambda,\bmphi) &=  \E_\lambda [\eta_l(\bmx_i,\bmbeta)]  - \bmphi_i,
\end{split}
\end{equation}
\noindent where $\nabla^{nat}$ denotes natural gradients\footnote{Natural gradient is the standard gradient permultiplied by the inverse of the Fisher information matrix. They advantage of these gradients is that they account for the Riemannian geometry of the parameter space \citep{amari1998natural}.}, and $\E_{\phi_i}[\cdot]$ and $\E_\lambda [\cdot]$ denote expectations with respect to $q(\bmz_i\given\bmphi_i)$ and $q(\bmbeta\given\bmlambda)$, respectively.



%where $\eta_\bmbeta (\bmalpha)$ and $\eta_{z_i}(\bmbeta)$ are the natural parameters of the conditional $\ln p(\bmbeta\given\bmalpha)$ and $\ln p(\bmz_i\given\bmbeta)$, respectively, following Equation \eqref{eq:exponentialform}. While $\E_q [\eta_\bmbeta (\bmx_i,\bmz_i)]$ and $\E_q [\eta_{z_i}(\bmx_i,\bmbeta)]$ are defined as in Equation~\eqref{eq:posteriorexponentialform}.

From the above gradients we can derive a coordinate ascent algorithm to optimize the ELBO function with the following coordinate ascent rules, 
\begin{eqnarray}\label{eq:CoordinateAscent}
\bmlambda^\star &=&  \arg\max_{\lambda} {\cal L} (\bmlambda, \bmphi) = \bmalpha + \sum_{i=1}^N  \E_{\phi_i} [t(\bmx_i,\bmz_i)]  \nonumber\\
\bmphi_i^\star &=& \arg\max_{\phi_i}  {\cal L} (\bmlambda, \bmphi) = \E_\lambda [\eta_l(\bmx_i,\bmbeta)].
\end{eqnarray}


By iteratively running the above updating equations, we are guranteed to (i) monotonically increased the ELBO function at every time step and (ii) to converge to stationary point of the ELBO function or, equivalently, the minimization function of Equation~\eqref{eq:VIKL}.

%While the natural gradient with respect to the variational parameter $\bmphi_i$ is computed as follows, 
%\begin{equation}\label{eq:gradELBOLocal}
%\begin{split}
%\nabla^{nat}_\bmphi_i {\cal L} = \E_q[\eta_{\bmz_i} (\bmbeta)] + \E_q [\eta_{\bmz_i} (\bmx_i)]  - \bmlambda,
%\end{split}
%\end{equation}

\begin{exmp}\label{example:PCA:VI}
For the PCA model depicted in Example \ref{example:PCA}, the variational distributions would be,
\begin{eqnarray*}
q(\bmbeta\given\bmlambda = (\bmmu_{\beta},  \mathbf{\Sigma}_{\beta})) = {\cal N}_{d\times k}(\bmmu_{\beta},  \mathbf{\Sigma}_{\beta})\\\\
q(\bmz\given\bmphi = \{\bmmu_{z,i}, \mathbf{\Sigma}_{z,i}\}_{i\in \{1,\ldots,N\}}) = \prod_{i=1}^N {\cal N}_{k}(\bmmu_{z,i},   \mathbf{\Sigma}_{z,i})
\end{eqnarray*}  

Given the above variational family, the coordinate updating equations derived from Equation~\eqref{eq:CoordinateAscent} can be written as follows \citep{bishop2006pattern},
\begin{eqnarray*}
\bmmu_{\beta}^\star &=& \big[\sum_{i=1}^N (\bmx_i - \bar{\bmx})\E[\bmz_i]^T\big]\mathbf{\Sigma}_{\beta}\\
\mathbf{\Sigma}_{\beta}^\star &=& \sum_{i=1}^N \E[\bmz_i\bmz_i^T] +  \sigma_x A)\\
\bmmu_{z}^\star &=& \sigma_x^2 \mathbf{\Sigma}_{z}^{-1}\bmmu_{\beta}^T(\bmx -\bar{\bmx})\\
\mathbf{\Sigma}_{z}^\star &=& \sigma_x^{-2}\bmmu_{\beta}^T\bmmu_{\beta} + \bmI
\end{eqnarray*}  
\noindent where $A$ is a diagonal matrix with elements $\alpha_i = \frac{d}{\bmmu_{\beta,i}^T\bmmu_{\beta,i}}$.
Again, we have a nice set of close-form equations which guarantees convergence to the solution of the inference problem. But we should note that this is possible due to the strong assumptions imposed to the probabilistic model and to the variational approximation family. 
%And the gradient wrt to the  variational parameters shown in Equation~\eqref{eq:gradELBO} can be computed by using the following equality,
%\begin{equation}
%\begin{split}
%\E_q[\eta_{z_i}(\bmbeta)]=\begin{bmatrix} ? \\ ? \end{bmatrix} & 
%\quad \E_q [\eta_\bmbeta (\bmx_i,\bmz_i)]=\begin{bmatrix} ? \\ ? \end{bmatrix} \\
%\E_q [\eta_{z_i}(\bmx_i,\bmbeta)]=\begin{bmatrix} ? \\ ? \end{bmatrix} & 
%\end{split}
%\end{equation}
\end{exmp}


%Other approaches exploit further the functional forms of the conjugate exponential models and allow to compute the 

%Moreover, the gradient can be computed locally, involves variables only in the Markov blanket of random variable. 
%with respect to the variational parameter $\phi_{i,j}$ can be computed as follows
%\begin{equation}\label{eq:gradELBO}
%\begin{split}
%\frac{\partial{\cal L}^{nat}}{\partial \phi_{i,j}} = &\E_q[\eta_{z_{i,j}}(\Pa(z_{i,j}))] \\
%\phantom{=}  &+ \sum_{Y\in \Ch(z_{i,j})}\E_q[\eta_{z_{i,j}}(Y,\Co_{z_{i,j}}(Y))) - \phi_{i,j}
%\end{split}
%\end{equation}
%\noindent where $\Co_{z_{i,j}}(Y)$ denotes the co-parents of  $z_{i,j}$ with respect to $Y$, which can be another local 
%hidden variable $z_{i,k}$ with $k\neq j$ or a global hidden variable $\beta_k$. This gradient can be similarly computed with respect to $\lambda_k$.


\subsection{Scalable Varitional Inference}\label{sec:ScalableVI}

Performing variational inference in big data sets (i.e. when N is a very large number) raises many challenges. Firstly, the model itself may not fit in memory, and, secondly, computing the ELBO's gradient wrt $\bmlambda$ 
depends linearly on the size of the data set (see Equation~\eqref{eq:gradELBO}), which can be prohibitively expensive in this case.  Stochastic Variational inference (SVI) \citep{HoffmanBleiWangPaisley13} is the most popular method for scaling VI to massive data sets, and relies on stochastic 
optimization techniques \citep{bottou2010large,robbins1951stochastic}. 

We start reparamerizing the ELBO's function ${\cal L}$ only in terms of the variational global parameters $\bmlambda$, by defining, 
\begin{equation}\label{eq:scalable:elbo}
{\cal L}(\bmlambda) = {\cal L}(\bmlambda,\bmphi^\star(\bmlambda)) 
\end{equation}
\noindent where $\bmphi^\star(\bmlambda)$ is defined as in Equation~\eqref{eq:CoordinateAscent}, i.e. it returns a local optimum of the local variational parameters for a given $\bmlambda$. By using the equality $\nabla^{nat}_\lambda {\cal L}(\bmlambda) = \nabla^{nat}_\lambda {\cal L}(\bmlambda,\bmphi^\star(\bmlambda))$  \citep{HoffmanBleiWangPaisley13},  the natural gradient wrt $\bmlambda$ can be computed as follows, 
\begin{equation}\label{eq:scalable:gradient}
\nabla^{nat}_\lambda {\cal L}(\bmlambda) = \bmalpha + \sum_{i=1}^N  \E_{\phi^\star} [t(\bmx_i,\bmz_i)]  - \bmlambda\\
\end{equation}

The key idea behind the stochastic variational method is to compute noise and unbiased estimates of the ELBO's gradient,  denoted by $\hat{\nabla}^{nat}_\lambda {\cal L}$,
by randomly selecting a  mini-batch of $M$ data samples, 
\begin{equation}\label{eq:scalable:gradientNoisy}
\begin{split}
\hat{\nabla}^{nat}_\lambda {\cal L} (\bmlambda) = \bmalpha + \frac{N}{M}\sum_{m=1}^M \E_{\phi^\star_i} [t (\bmx_{i_m},\bmz_{i_m})]  - \bmlambda,
\end{split}
\end{equation}
\noindent where $i_m$ is the variable index form the subsampled mini-batch. This is an unbiased estimate because $\E[\hat{\nabla}^{nat}_\lambda {\cal L}] = \nabla^{nat}_\lambda {\cal L}$. 

According to stochastic optimization theory \citep{robbins1951stochastic}, the ELBO can be maxizimed by following noisy estimates of the gradient, 
\begin{equation}\label{eq:gradELBONoisy}
\begin{split}
\bmlambda^{t+1} = \bmlambda^t + \rho_t \hat{\nabla}^{nat}_\lambda {\cal L}(\bmlambda^t),
\end{split}
\end{equation}
\noindent if the learning rate $\rho_t$ satisfies the Robbins-Monro conditions (i.e. $\sum_{t=1}^\infty \rho_t = \infty$ and $\sum_{t=1}^\infty \rho^2_t<\infty$), and the above updating equation is guarantee to converge to a stationary point of the ELBO function. 

The size of the mini-batch is chosen to be $S<<M$ to reduce the computational complexity of computing the gradient, and with $S>1$ in order to reduce the variance in the estimate of the gradient. The optimal value is used to be problem dependent. 

Alternative ways to scale up variational inference in conjugate exponential models involve the use of distributed computing clusters. For example, in \citep{masegosa2017scaling} the data set is assumed to be stored among different machines. Then the problem of computing the ELBO's gradient given in Equation~\eqref{eq:gradELBO} is scaled up by distributing the computation of the gradient  $\nabla^{nat}_{\phi_i}{\cal L} (\bmlambda,\bmphi)$ . So each machine computes this term for those samples that are locally stored. Finally, all the terms are sent to a master node which aggregates them and compute the gradient $\nabla^{nat}_\lambda {\cal L} (\bmlambda,\bmphi)$ (see Equation~\eqref{eq:gradELBO}). 


\section{Probabilistic Models with Deep Neural networks}\label{sec:modelsDNNs}
\subsection{Introduction}
LVMs has been usually restricted to belong to the conjugate exponential family because, in this case, inference was feasible (and scalable). But recent advances in variational inference (which will be revised in Section \ref{sec:variational}) is inspiring many recent work about extending LVMs with DNNs. Variational Auto-encoders (VAE) \citep{kingma2013auto,doersch2016tutorial} are probably the most influential work combining LVMs and deep neural netorwks. VAEs extend the classic techine of principal component analysis (PCA) \citep{jolliffe2011principal} for data representation in lower-dimensional spaces. More precisely, \cite{kingma2013auto} extends the probabilistic version of the PCA model \citep{tipping1999probabilistic} where the relationship between the low-dimensional representation and the observed data is governed by a DNN, i.e. a highly non-linear function, as opposed to the standard linear assumptions of the basic version of the PCA model. This new models were able to capture much more compact low-dimensional representation specially in cases where data was highly-dimensional and complex\footnote{Technically, it refers to high-dimensional data which ''lives'' in a low-dimensional manifold \citep{pless2009survey}.}. As it is the case of image data \citep{kingma2013auto,kulkarni2015deep,gregor2015draw,sohn2015learning,pu2016variational}, text data \citep{semeniuta2017hybrid}, audio data \citep{hsu2017learning}, chemical molecules \citep{gomez2018automatic}, etc.

As commented above, VAEs have given raised to a pletora of extensions of classic LVMs to their \emph{deep countepart}, which mainly are the ones we cover in this work. \cite{johnson2016composing} contains different examples of this approach an extends Gaussian mixture models, latent linear dynamical systems and  latent switching linear dynamical systems with non-linear relationships modeled by DNNs. \cite{linderman2016recurrent} extends hidden semi-Markov models with recurrent neural networks. \cite{zhou2015poisson,card2017neural} extends popular LDA models \citep{blei2003latent} for uncovering topics in text data. Many other works are following this same trend \citep{chung2015recurrent,jiang2016variational,xie2016unsupervised,louizos2017causal}.


LVMs with DNNs can also be found in the literature under the name of deep generative models \citep{hinton2009deep,hinton2012practical,goodfellow2014generative,salakhutdinov2015learning}. These models highlight their the capacity to generate data samples using probabilistic constructs that include DNNs. This new capacity has also provoked a strong impact within the deep learning community, and has opened the possiblity of dealing with unsupervised learning problems, as opposed to the \textit{classic deep learning methods} which were mainly focused on supervised learning settings. In any case, this active area of research is out of the scope of this paper and contains many alternative models which do not fall within the category of models explored in this work \citep{goodfellow2014generative}. 


%\subsection{LVMs with DNNs}

%How to choose the right family and architecture of DNNs is beyond the scope of this paper.  [] contains a general and recent overview of deep neural networks. The optimal family and architecture depends of the specific relationships and the kind of data we want to model. But the definition of a DNN as a deterministic non-linear function is general enough to cover the vast majority of the current uses of DNNs within current probabilistic modeling approaches. 

\subsection{Model Definition}

We consider here a deep neural network \citep{goodfellow2016deep} as a deterministic non-linear function, denoted by $f(\cdot; \bmbeta)$, and which is parameterized by a parameter vector $\bmbeta$. A \emph{latent variable model with DNNs} has the same structure that one provided in Figure \ref{fig:plateModel}, but with the following conditional distributions forms,
\begin{eqnarray}\label{eq:dnnexponentialform}
\ln p(\bmbeta) &=& \ln h(\bmbeta) + \bmalpha^T t(\bmbeta) - a_g(\bmalpha)\nonumber\\
\ln p(\bmz_i|\bmbeta) &=& \ln h(\bmz_i)  + \eta_z(\bmbeta)^T t(\bmz_i) - a_z(\eta_z(\bmbeta))\nonumber\\
\ln p(\bmx_i|\bmz_i,\bmbeta) &=& \ln h(\bmx_i)  + \eta_x(f(\bmz_i;\bmbeta))^T t(\bmx_i) - a_x(f(\bmz_i;\bmbeta)),.
\end{eqnarray}

The main difference with respect to a standard LVMs described in Section \ref{sec:LVM} (Equation~\ref{eq:model}) is the conditional distribution over the observations $\bmx_i$ given the local hidden variables $\bmz_i$ and the global parameters $\bmbeta$. Now this conditional relationship is governed by the DNN encoded in the (non-linear) function $f$, which is now parameterized by $\bmbeta$. A graphical description of this new model can be found in Figure \ref{fig:DNNModel}.

\begin{figure}
\begin{center}
\includegraphics[scale = 0.4]{./figs/DNNModel}
\end{center}
\caption{\label{fig:DNNModel} Core of the probabilistic model with DNNs examined in this paper. See \secref{sec:modelsDNNs} for details.}
\end{figure}

Models with conditional distributions as defined in Equation~\eqref{eq:dnnexponentialform} does not belong to the exponential family because they can not be represented in the forms given by Equations~\eqref{eq:jointexponentialform} and \eqref{eq:posteriorexponentialform}.  In consequence, the variational inference techniques detailed in Sections \ref{sec:VI} and \ref{sec:ScalableVI} do not apply here.

Deep exponential family models  \citep{ranganath2015deep} would be a straightforward extension of this model family which is not covered in this paper.  It includes different hierarchies of latent variables which gives rise to a more expressive model family. But all the inference methods visited in this work would apply to these more complex models with minor adaptations. 
\vspace{2cm}
\begin{exmp}\label{example:vae}
The generative part of a VAE model \citep{kingma2013auto} can be described as follows, 
\begin{equation}\label{eq:vae}
\begin{split}
\bmbeta_\mu, \bmbeta_\sigma \sim \calN_R (0,\bmI\sigma_\bmbeta)\nonumber\\ 
\bmz_i \sim \calN_K (0,\bmI\sigma_\bmz)\nonumber\\ 
\bmx_i \sim \calN_D (\mu(\bmz_i;\bmbeta_\mu), \sigma(\bmz_i;\bmbeta_\sigma)),
\end{split}
\end{equation}
\noindent where $\mu(\cdot;\bmbeta_\mu)$ and $\sigma(\cdot;\bmbeta_\sigma)$ are DNNs functions with input $\bmz_i$ and output the mean vector and the covariance matrix of $\bmx_i$, respectively. 

This model is quite similar to the PCA model presented in Example~\ref{example:PCA}. The main difference comes from the conditional distribution of $\bmx_i$. In the PCA model, the mean of the Normal distribution of $\bmx_i$ depends linearly of $\bmz_i$ through $\bmbeta$. In the VAE model, the mean (and the variance) depends of $\bmz_i$ through a DNN parametrized by $\bmbeta$. It easy to see that this model belongs to the model family described by Equations~~\eqref{eq:dnnexponentialform}.

%A VAE falls inside the general models class described in this section. In this case, $\bmalpha=\sigma_z$, $\bmbeta=\emptyset$ and $p(\bmz_i|\bmbeta)$ is a Normal distribution which belongs to the exponential family. Finally, the mean and the variance (and, hence, the natural parameters) of the Normal distribution of $\bmx_i$ depends of $\bmz_i$ through a DNN with parameters $\bmbeta = (\bmbeta_\mu, \bmbeta_\sigma)$. 
\end{exmp}



%We will probably see more works extending other LVMs following this approach in the coming years. 

%\subsection{Probabilistic Simulators with DNNs}




==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


